Submodularity in Input Node Selection for Networked Systems

Networked systems are systems of interconnected components, in which the dynamics of each component are influenced by the behavior of neighboring components. Examples of networked systems include biological networks, critical infrastructures such as power grids, transportation systems, and the Internet, and social networks. The growing importance of such systems has led to an interest in control of networks to ensure performance, stability, robustness, and resilience. A widely-studied method for controlling networked systems is to directly control a subset of input nodes, which then steer the remaining nodes to their desired states. This article presents submodular optimization approaches for input node selection in networked systems. Submodularity is a property of set functions that enables the development of computationally tractable algorithms with provable optimality bounds. For a variety of physically relevant systems, the physical dynamics have submodular structures that can be exploited to develop efficient input selection algorithms. This article will describe these structures and the resulting algorithms, as well as discuss open problems.

==> Figures.tex <==
\newpage
\begin{figure}[!ht]
\centering
\includegraphics[width=4in]{Figures/set_cover_example.eps}
\caption{Submodularity of the set cover problem. Define $A$ to be a finite set and $R_{1},\ldots,R_{n}$ to be  subsets of $A$. The function $f(S)$ is given by $f(X) = \left|\bigcup_{i \in X}{R_{i}}\right|$, where $| \cdot |$ denotes cardinality of a set. In this example, $A = \{a_{1},\ldots,a_{8}\}$, $R_{1},\ldots,R_{4}$ are defined as shown, $S = \{1\}$, $T = \{1,3,4\}$, and $v=2$. All elements contained in $v$ are already contained in $T$, and hence adding $v$ to $T$ results in no incremental increase in $f$.}
\label{fig:set_cover}
\end{figure}

\newpage
\begin{figure}[!ht]
\centering
\includegraphics[width=5in]{Figures/submod_example3.eps}
%\caption{Example of submodularity. Each node (grey cylinder) has a coverage area, equal to the area that the node can monitor. The goal of maximizing the coverage area is captured by the objective function $f(S)$, which is equal to the total area covered by a set of sensors denoted $S$. (a) Incremental increase in coverage area from adding a node $v$ (coverage area in green) to the set $S$ (coverage area in blue). (b) Incremental increase in coverage area from adding node $v$ to the set $T$ (coverage area in yellow), which contains $S$ as a subset. The incremental increase from adding $v$ to $T$ is smaller than the incremental increase from adding $v$ to $S$, since most of node $v$'s coverage area is already covered by the nodes in $T$. Hence $f(S)$ is a submodular function of $S$.}
\caption{Example of submodularity. Each sensor (grey cylinder) has a coverage area, equal to the area that the sensor can monitor. The goal is to monitor the rectangular region by selecting a subset of active sensors. The function $f(S)$ is equal to the total area covered by the set of sensors, denoted $S$. Solid blue circles represent the coverage areas of sensors that are active. The dashed lines indicate the coverage area of the sensor $n_{5}$. (a) Incremental increase in coverage area from adding $n_{5}$ to the set of active sensors $S = \{n_{1}, n_{2}, n_{3}\}$. (b) Incremental increase in coverage area from adding $n_{5}$ to the set $T = \{n_{1}, n_{2}, n_{3}, n_{7}\}$. The incremental increase $f(T \cup \{n_{5}\}) - f(T)$ from adding $n_{5}$ to $T$ is smaller than the incremental increase from adding $n_{5}$ to $S$, since most of $n_{5}$'s coverage area is already covered by the sensors in $T$. Hence $f$ is a submodular function.}
\label{fig:submod}
\end{figure}

\newpage
\begin{figure}[!ht]
\centering
\includegraphics[width=4in]{Figures/transversal-2.eps}
\caption{A set $X$ is independent in a transversal matroid if there is a matching where each node in $X$ is matched to exactly one node in $W$. In this example, the set $X = \{1, 2, 5\}$ is independent, since there is a matching in which each node in $\{w_{i} : i \in X\}$ is matched to exactly one neighbor in $U$. Note that this matching is not unique: for example, $w_{2}$ could be matched to $u_{2}$, $u_{3}$, or $u_{4}$.  The set $X^{\prime} = \{3, 5\}$ is not independent, since nodes $w_{3}$ and $w_{5}$ can only be matched to the same node  $u_{6}$.} %and hence there is no matching in which both $w_{3}$ and $w_{5}$ are matched.}
\label{fig:transversal}
\end{figure}

\newpage
 \begin{figure}[!ht]
 \centering
 $\begin{array}{cc}
 \includegraphics[width=3in]{Figures/L_ff_illustration.eps} &
 \includegraphics[width=3in]{Figures/L_ff_rw.eps} \\
 \mbox{(a)} & \mbox{(b)}
 \end{array}$
 \caption{Description of the connection between the inverse Laplacian and a random walk on the graph. (a) Illustration of the vector $v^{\ast}$ used to compute the error due to noise at node $u$, equal to $(L_{ff}^{-1})_{uu}$,  when $S = \{6,8\}$. (b) Connection to a random walk. The variable $\tilde{v}_{i}$ is equal to the probability that a walk originating at $i$ reaches $u$ before $S$ under a random walk with transition matrix $P$. $P_{21}$, $P_{23}$, and $P_{25}$ denote the transition probabilities of the walk. It can be shown using the Maximum Principle that $v^{\ast} = \tilde{v}$.}
 \label{fig:rw_explanation}
 \end{figure}
 
 \newpage
 \begin{figure}[!ht]
\centering
$\begin{array}{ccc}
\includegraphics[width=2in]{Figures/commute_supermodular1.eps} &
\includegraphics[width=2in]{Figures/commute_supermodular2.eps} &
\includegraphics[width=2in]{Figures/commute_supermodular3.eps} \\
\mbox{(a)} & \mbox{(b)} & \mbox{(c)}
\end{array}$
\caption{Illustrations of the supermodularity of commute time. (a) If the walk reaches $j$ before $T$, then it automatically reaches $j$ before $S$, implying that $\tau_{j}(T) \subseteq \tau_{j}(S)$. (b) When a walk starting at $j$ reaches $S$ before $u$, the time for the walk to start at $j$, reach $S$, and then reach $u$ ($U_{jSu}$) is equal to the corresponding time $U_{jTu}$ for set $T$. (c) The case where $U_{jSu} > U_{jTu}$. In this case, the walk reaches $T \setminus S$ and then reaches node $u$ before reaching any node in $S$.}
\label{fig:commute_supermodular}
\end{figure}

\newpage
\begin{figure}[!ht]
\centering
$\begin{array}{ccc}
\includegraphics[width=2in]{Figures/noise_example1.eps} &
\includegraphics[width=2in]{Figures/noise_example2.eps} &
\includegraphics[width=2in]{Figures/noise_example3.eps} \\
\mbox{(a)} & \mbox{(b)} & \mbox{(c)} 
\end{array}$
\caption{Example of input selection for robustness to noise. (a) Initial network topology with no input nodes. (b) Input selected at first iteration of greedy algorithm. Since all nodes will provide the same error due to noise, the selection of the first input node is arbitrary. (c) Input selected at second iteration. The greedy algorithm will select node $n_{6}$, leading to an input set $\{n_{1},n_{6}\}$.}
\label{fig:noise_example}
\end{figure}

\newpage
\begin{figure}[!ht]
\centering
\includegraphics[width=2.5in]{Figures/containment.eps}
\caption{Containment in a networked system. The non-input node positions (purple circles) are in the convex hull of the positions of the input nodes (green triangles).}
\label{fig:containment}
\end{figure}
 
